Cosmetic operations and Khovanov multicurves

We prove an equivariant version of the Cosmetic Surgery Conjecture for strongly invertible knots. Our proof combines a recent result of Hanselman with the Khovanov multicurve invariants $\widetilde{\operatorname{Kh}}$ and $\widetilde{\operatorname{BN}}$. We apply the same techniques to reprove a result of Wang about the Cosmetic Crossing Conjecture and split links. Along the way, we show that $\widetilde{\operatorname{Kh}}$ and $\widetilde{\operatorname{BN}}$ detect if a Conway tangle is split.

==> PSTricks/PSTricks-pics-header.tex <==
\usepackage[top=1in, bottom=1.25in, marginparwidth=1in, inner=1in, outer=1in]{geometry}

\usepackage{lmodern}
\usepackage[T2A,T1]{fontenc} % T2A for Cyrillic letters
\usepackage{bm}
\pagestyle{empty}

\usepackage{graphicx}
\usepackage{xcolor}
\colorlet{myblue}{black}
\colorlet{gold}{yellow!90!black!70!red}
\colorlet{darkgreen}{green!70!black}
\colorlet{lightgreen}{green!50!white}
\colorlet{lightred}{red!30!white}
\colorlet{lightblue}{blue!50!white}

\usepackage{setspace} 
\singlespacing
\sloppy
\raggedbottom

\usepackage{pstricks,pstricks-add}
\usepackage[crop=off,runs=1]{auto-pst-pdf}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\mathtoolsset{mathic=true}
\usepackage{nicefrac}

\newcommand{\m}{\operatorname{m}}% old mirror command
\input{../0_notation.tex}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[cmtip,all]{xy}
\newcommand{\longsquiggly}{\xymatrix{{}\ar@{~>}[r]&{}}}
\newcommand{\myarrow}[1][1cm]{\mathrel{%
		\hbox{\usefont{U}{lasy}{m}{n}\symbol{40}}%
		\mkern-4mu%
		\hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
		\mkern-4mu%
		\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\usepackage{stackengine} %% this is for nodes with multiline-labels
\setstackEOL{\\}

% predefined functions for morphism classification

\newcommand{\dotcircle}{\pscircle[linestyle=dotted,dotsep=1pt](0,0){2}}
\newcommand{\cobcircle}{\pscircle[linewidth=0.25pt](0,0){2}}

\makeatletter
\def\bpt{\pst@object{bpt}}
\def\bpt@i#1(#2){%
	\begin@OpenObj%
	\psdot[dotstyle=asterisk,dotsize=4pt,dotangle=#1](#2)
	\psdot[dotsize=0.8pt](#2)
	\end@OpenObj%
}
\def\pswrap{\pst@object{pswrap}}
\def\pswrap@i#1(#2)#3{%
	\begin@OpenObj%
	\rput{#3}(0,0){%
		\parametricplot[#1,plotstyle=curve,plotpoints=300,algebraic]{0}{#2}%
		{10*(1-(t/5)^(1/2)/2)*cos(2*Pi*t/4)|10*(1-(t/5)^(1/2)/2)*sin(2*Pi*t/4)}%
	}
	\end@OpenObj%
}
\def\pswrapn{\pst@object{pswrapn}}
\def\pswrapn@i#1(#2)#3{%
	\begin@OpenObj%
	\rput{#3}(0,0){%
		\parametricplot[#1,plotstyle=curve,plotpoints=300,algebraic]{0}{#2}%
		{10*(1-((#2-t)/5)^(1/2)/2)*cos(2*Pi*(#2-t)/4)|10*(1-((#2-t)/5)^(1/2)/2)*sin(2*Pi*(#2-t)/4)}%
	}
	\end@OpenObj%
}
\def\pswrapend{\pst@object{pswrapend}}
\def\pswrapend@i#1(#2)#3{%
	\begin@ClosedObj%
	\rput{#3}(0,0){%
		\psline[arrows=->,#1]%
		(!10 1 #2 5 div 1 2 div exp 2 div sub mul 360 #2 mul 4 div cos mul 10 1 #2 5 div 1 2 div exp 2 div sub mul 360 #2 mul 4 div sin mul)(!10 360 #2 mul 4 div cos mul 10 360 #2 mul 4 div sin mul)
	}
	\end@ClosedObj%
}
\def\psMorBoundary{\pst@object{psMorBoundary}}
\def\psMorBoundary@i#1{%
	\begin@ClosedObj%
	\rput*{#1}(0,0){
		\pscustom*[linecolor=lightred,linewidth=0pt]{
			\psarc(0,0){10}{-20}{20}
			\psline(10;20)(12;20)
			\psarcn(0,0){12}{20}{-20}
			\psline(12;-20)(10;-20)
		}
		\psarc(0,0){10}{-20}{20}
		\psline(9.7;0)(10.3;0)
	}
	\end@ClosedObj%
}
\def\psLagwrap{\pst@object{psLagwrap}}
\def\psLagwrap@i#1#2(#3)#4#5{%
	% #1 is a scalar, usually 0.5, which is the maximal radius 
	% #2 is an angle, which rotates the picture
	% #3 is a coordinate x,y
	% #4 is a colour
	% #5 is a number and defined the start of the curve (usually 0)
	\begin@ClosedObj%
	\rput{#2}(#3){
		\parametricplot[linecolor=#4,plotstyle=curve,plotpoints=200]{#5}{10}{%
			0.14 #1 0.14 sub 1 t t mul add div add 360 t mul cos mul
			0.14 #1 0.14 sub 1 t t mul add div add 360 t mul sin mul
		}}
	\end@ClosedObj%
}
\def\psLi{%
	\psrotate(0,0){45}{
		\dotcircle
		%\psdot[linecolor=red](0,2)
		\rput(0,2){$\ast$}
		\pscustom{
			\psline(0,2)(0,1)
			\psarcn(-1,1){1}{0}{-90}
			\psline(-1,0)(-2,0)
		}%
		\pscustom{
			\psline(0,-2)(0,-1)
			\psarcn(1,-1){1}{180}{90}
			\psline(1,0)(2,0)
		}%
	}
}
\def\psLo{%
	\psrotate(0,0){45}{
		\dotcircle
		%\psdot[linecolor=red](0,2)
		\rput(0,2){$\ast$}
		\pscustom{
			\psline(0,2)(0,1)
			\psarc(1,1){1}{-180}{-90}
			\psline(1,0)(2,0)
		}%
		\pscustom{
			\psline(0,-2)(0,-1)
			\psarc(-1,-1){1}{0}{90}
			\psline(-1,0)(-2,0)
		}%
	}
}	
\makeatother



\newlength{\stringwidth}
\setlength{\stringwidth}{1.5pt}
\newlength{\stringwhite}
\setlength{\stringwhite}{5.5pt}

\newlength{\stringwidthThick}
\setlength{\stringwidthThick}{2.5pt}
\newlength{\stringwhiteThick}
\setlength{\stringwhiteThick}{7.5pt}


\newpsstyle{para}{linestyle=dotted,dotsep=1pt,linewidth=\stringwidth,linecolor=gray}
\newpsstyle{parawide}{linestyle=dotted,linewidth=\stringwidth,linecolor=gray}
\newpsstyle{curveblue}{linewidth=1pt,linecolor=blue}
\newpsstyle{curvered}{linewidth=1pt,linecolor=red}


\newcommand{\mysquare}{%
	\psline[style=para](4,4)(4,-4)
	\psline[style=para](4,-4)(-4,-4)
	\psline[style=para](-4,-4)(-4,4)
	\psline[style=para](-4,4)(4,4)
	\pscircle[fillcolor=white,fillstyle=solid](4,4){0.5}
	\pscircle[fillcolor=white,fillstyle=solid](-4,4){0.5}
	\pscircle[fillcolor=white,fillstyle=solid](-4,-4){0.5}
	\pscircle[fillcolor=white,fillstyle=solid](4,-4){0.5}
}
